Microarchitectural Security of AWS Firecracker VMM for Serverless Cloud Platforms

Firecracker is a virtual machine manager (VMM) built by Amazon Web Services (AWS) for serverless cloud platforms, services that run code for end users on a per-task basis, automatically managing server infrastructure. Firecracker provides fast and lightweight VMs and promises a combination of the speed of containers, typically used to isolate small tasks, and the security of VMs, which tend to provide greater isolation at the cost of performance. This combination of security and efficiency, AWS claims, makes it not only possible but safe to run thousands of user tasks from different users on the same hardware, with the host system frequently switching between active tasks. Though AWS states that microarchitectural attacks are included in their threat model, this class of attacks directly relies on shared hardware, just as the scalability of serverless computing relies on sharing hardware between unprecedented numbers of users. In this work, we investigate how secure Firecracker is against microarchitectural attacks. First, we review Firecracker's stated isolation model and recommended best practices for deployment, identify potential threat models for serverless platforms, and analyze potential weak points. Then, we use microarchitectural attack proof-of-concepts to test the isolation provided by Firecracker and find that it offers little protection against Spectre or MDS attacks. We discover two particularly concerning cases: 1) a Medusa variant that threatens Firecracker VMs but not processes running outside them, and is not mitigated by defenses recommended by AWS, and 2) a Spectre-PHT variant that remains exploitable even if recommended countermeasures are in place and SMT is disabled in the system. In summary, we show that AWS overstates the security inherent to the Firecracker VMM and provides incomplete guidance for properly securing cloud systems that use Firecracker.

==> figures/background/intel-amd-virtualization.tex <==
\begin{tikzpicture}[
    common/.style = {
        minimum height=.75cm,
        node distance=0cm
    },
    small layer/.style = {
        common,
        minimum width=.135\textwidth,
    },
    large layer/.style={
        common,
        minimum width=.3\textwidth,
    },
    gate/.style = {
        draw,
        fill=niceyellowborder,
        node distance=0cm,
        minimum width=.05\textwidth,
    },
    vm/.style= {
        -,
        draw,
        fill=plotorange!80!white
    },
    vmm/.style = {
        -,
        draw,
        fill=nicegreenborder
    },
    kern/.style = {
        -,
        draw,
        fill=plotblue!80!white
    }
]

%%%%%%%%%%%%%%
%%% CPU
%%%%%%%%%%%%%%
\node[large layer](cpu) {};
\path[kern]    (cpu.south east)
            -- (cpu.north east)
            -- (cpu.north west)
            -- (cpu.south west)
            -- cycle;
\path[kern]    (cpu.south east)
            -- ([xshift=4em,yshift=4em]cpu.south east)
            -- ([xshift=4em,yshift=4em]cpu.north east)
            -- (cpu.north east)
            -- (cpu.south east)
            -- cycle;
\path[kern]    (cpu.north east)
            -- ([xshift=4em,yshift=4em]cpu.north east)
            -- ([xshift=4em,yshift=4em]cpu.north west)
            -- (cpu.north west)
            -- (cpu.north east)
            -- cycle;
\node[] at (cpu) {CPU};

%%%%%%%%%%%%%%%
%%% Host Kernel
%%%%%%%%%%%%%%%
\node[large layer,above=of cpu.north west,anchor=south west](knl){};
\path[kern]    (knl.south east)
            -- (knl.north east)
            -- (knl.north west)
            -- (knl.south west)
            -- cycle;
\path[kern]    (knl.south east)
            -- ([xshift=4em,yshift=4em]knl.south east)
            -- ([xshift=4em,yshift=4em]knl.north east)
            -- (knl.north east)
            -- cycle;
\path[kern]    (knl.north east)
            -- ([xshift=4em,yshift=4em]knl.north east)
            -- ([xshift=4em,yshift=4em]knl.north west)
            -- (knl.north west)
            -- (knl.north east)
            -- cycle;
\node[] at (knl) {Host Kernel};

%%%%%%%%%%%%%%%%
%%% Guest Kernel
%%%%%%%%%%%%%%%%
\node[small layer,above=of knl.north west,anchor=south west](vm){};
\foreach \x/\y in {3/4,1.5/2.5,0/1}{
    \path[-,draw,fill=plotorange!80!white]
           ([xshift=\x em,yshift=\x em]vm.south east)
        -- ([xshift=\y em,yshift=\y em]vm.south east)
        -- ([xshift=\y em,yshift=\y em]vm.north east)
        -- ([xshift=\x em,yshift=\x em]vm.north east)
        -- cycle;
    \path[-,draw,fill=plotorange!80!white]   
           ([xshift=\x em,yshift=\x em]vm.south east)
        -- ([xshift=\x em,yshift=\x em]vm.south west)
        -- ([xshift=\x em,yshift=\x em]vm.north west)
        -- ([xshift=\x em,yshift=\x em]vm.north east)
        -- cycle;
}
\node[] at (vm) {Guest Kernel};

%%%%%%%%%%%%%%%
%%% Guest App
%%%%%%%%%%%%%%%
\node[small layer,above=of vm.north west,anchor=south west](app){};
\foreach \x/\y in {3/4,1.5/2.5,0/1}{
    \path[vm]  ([xshift=\x em,yshift=\x em]app.south east)
            -- ([xshift=\y em,yshift=\y em]app.south east)
            -- ([xshift=\y em,yshift=\y em]app.north east)
            -- ([xshift=\x em,yshift=\x em]app.north east)
            -- cycle;
    \path[vm]  ([xshift=\x em,yshift=\x em]app.north east)
            -- ([xshift=\y em,yshift=\y em]app.north east)
            -- ([xshift=\y em,yshift=\y em]app.north west)
            -- ([xshift=\x em,yshift=\x em]app.north west)
            -- cycle;
    \path[vm]  ([xshift=\x em,yshift=\x em]app.south east)
            -- ([xshift=\x em,yshift=\x em]app.south west)
            -- ([xshift=\x em,yshift=\x em]app.north west)
            -- ([xshift=\x em,yshift=\x em]app.north east)
            -- cycle;
}
\node[] at (app) {App};

%%%%%%%%%%%%%%%
%%% VMM
%%%%%%%%%%%%%%%
\node[small layer,above=of knl.north east,anchor=south east](vmm){};
\foreach \x/\y in {3/4,1.5/2.5,0/1}{
    \path[vmm] ([xshift=\x em,yshift=\x em]vmm.south east)
            -- ([xshift=\y em,yshift=\y em]vmm.south east)
            -- ([xshift=\y em,yshift=\y em]vmm.north east)
            -- ([xshift=\x em,yshift=\x em]vmm.north east)
            -- cycle;
    \path[vmm] ([xshift=\x em,yshift=\x em]vmm.north east)
            -- ([xshift=\y em,yshift=\y em]vmm.north east)
            -- ([xshift=\y em,yshift=\y em]vmm.north west)
            -- ([xshift=\x em,yshift=\x em]vmm.north west)
            -- cycle;
    \path[vmm] ([xshift=\x em,yshift=\x em]vmm.south east)
            -- ([xshift=\x em,yshift=\x em]vmm.south west)
            -- ([xshift=\x em,yshift=\x em]vmm.north west)
            -- ([xshift=\x em,yshift=\x em]vmm.north east)
            -- cycle;
}
\node[] at (vmm) {VMM};

%%%%%%%%%%%%%%%
%%% KVM
%%%%%%%%%%%%%%%
\node[gate] (kvm) at ([yshift=-.4em]vmm.south) {KVM};
\path[-stealth] (kvm.south) edge[bend left=35] (vm.south);

%%%%%%%%%%%%%%%
%%% Rings
%%%%%%%%%%%%%%%
\path[draw,very thick,dashed]
    ([xshift=-5  em]vm.north west) -- ([xshift=  .5em]vm.north east)
    ([xshift=  .5em]vm.north east) -- ([xshift=  .5em]vm.south east)
    ([xshift=  .5em]vm.south east) -- ([xshift= 5  em]vmm.south east);
\node[] at ([xshift=-3em]knl.west) {Ring 0};
\node[] at ([xshift=-3em]app.west) {Ring 3};

%%%%%%%%%%%%%%%
%%% Modes
%%%%%%%%%%%%%%%
\node[plotblue!80!white,rotate=45] at ([xshift=2.5em,yshift=1.5em]cpu.south east) {\bfseries Kernel Mode};
\node[nicegreenborder] at ([xshift=4em,yshift=4.7em]vmm.north) {\bfseries User Mode};
\node[plotorange!80!white,rotate=45] at ([xshift=1.5em,yshift=2.5em]app.north west) {\bfseries Guest Mode};

\end{tikzpicture}


==> figures/background/kvm-guest-execution.tex <==
\begin{tikzpicture}[
    ->=stealth,
    size/.style = {
        text centered
    },
    process/.style = {
        size,
        rectangle,
        minimum height=1.5cm,
        text width=1.4cm,
        draw=niceorangeborder,
        fill=niceorangefill
    },
    decision/.style = {
        size,
        diamond,
        aspect=2,
        text width=1.4cm,
        minimum width=2.7cm,
        inner sep=0,
        draw=nicegreenborder,
        fill=nicegreenfill
    }
]

%%% Headings
\node[
] (km) {Kernel mode};
\node[
    left=1.5cm of km
] (um) {User mode};
\node[
    right=1.5cm of km
] (gm) {Guest mode};

%%% Nodes
\node[
    process,
    below=.25cm of um
] (igei) {ioctl: Start Guest};
\node[
    process,
    at={([yshift=-1em]km |- igei)},
    anchor=north
] (egm) {Enter Guest Mode};
\node[
    process,
    at={([yshift=-1em]gm |- egm)},
    anchor=north
] (enigm) {Execute natively in Guest Mode};
\node[
    process,
    at={([yshift=-1em]km |- enigm)},
    anchor=north,
    text width=1.5cm
] (he) {Handle Exit};
\node[
    decision,
    below=.5cm of he
] (io) {I/O?};
\node[
    decision,
    below=.5cm of io
] (sp) {Signal Pending?};
\node[
    process,
    at={(um |- sp)}
] (hio) {Handle I/O};

%%% Arrows
\draw[->] (igei.east)   -| (egm.north);
\draw[->] (egm.east)    -| (enigm.north);
\draw[->] (enigm.south) |- (he.east);
\draw[->] (he.south)    -- (io.north);
\draw[->] (io.south)    -- node[near start,left] {No}  (sp.north);
\draw[->] (io.west)     -| node[near start,above] {Yes} (hio.north);
\draw[->] (sp.west)     -- node[near end,  above] {Yes} (hio.east);
\draw[->] (sp.south)    -- ++(0,-1em)
                        -- node[near start,above] {No}  ++(-4.5em,0)
                        |- (egm.west);
\draw[->] (hio.west)    -- ++(-1em,0)
                        |- (igei.west);

%%% Dotted lines
\path (um.north) -- node[midway] (ll) {} (km.north);
\path (km.north) -- node[midway] (rr) {} (gm.north);
\draw[-,dashed] (ll) -- ([yshift=-1.5em]ll |- sp.south);
\draw[-,dashed] (rr) -- ([yshift=-1.5em]rr |- sp.south);

\end{tikzpicture}

==> figures/mds_genealogy.tex <==
\begin{tikzpicture}

\node (mfbds) at (0,0){MFBDS};
\node (mlpds) at (2,0){MLPDS};
\node (msbds) at (4,0){MSBDS};


\end{tikzpicture}

==> figures/mds_genealogy_old.tex <==
\begin{tikzpicture}
\node{MDS attacks} [sibling distance = 4 cm]
    child {node[text width=1.5cm, align=center] (mfbds) {RIDL\\(MFBDS)} [sibling distance = 2 cm, level distance = 2 cm]
        child {node[text width=1.5cm, align=center] (verw) {VERW bypass} edge from parent [dashed]}%  node [left, align=center] {bug in\\buffer\\overwrite}}
        child {node[text width=1.5cm, align=center] (l1des) {L1DES} edge from parent [dashed]}% node [right] {L1 cache eviction}}
        child {node[text width=1.5cm, align=center] (taa) {TAA} edge from parent [dashed]}% node [right] {TSX}}
        }
    child {node[text width=1.5cm, align=center] (msbds) {Fallout\\(MSBDS)}}
    child {node[text width=1.5cm, align=center] (mlpds) {RIDL\\(MLPDS)}}
    child {node[text width=1.5cm, align=center] (vrs) {VRS}}
    ;
    
\draw[dashed] (msbds) -- (taa);
\draw[dashed] (l1des) -- (taa)
\draw[dashed (]

\end{tikzpicture}

==> tables/medusa/medusa-all-disabled.tex <==
\begin{tabular}{c  c c  c c }
    \toprule
    & \multicolumn{2}{c}{\textbf{Block Write}} & \multicolumn{2}{c}{\repmov} \\
    \cmidrule(rl){2-3} \cmidrule(rl){4-5}
    \textbf{Leak} & Bare Metal & Firecracker & Bare Metal & Firecracker \\
    \midrule
    Cache Indexing & \xmark & \cmark & \cmark & \xmark \\
    Unaligned Store-to-Load & \cmark & \cmark & \cmark & \cmark \\
    Shadow \repmov & \xmark & \xmark & \cmark & \cmark \\
    \bottomrule
\end{tabular}

==> tables/spectre/bm-spectre-pocs-protected.tex <==
\begin{tabular}{cccccc}
    \toprule
                                   &              & PHT    & BTB        & RSB    & STL    \\
    \midrule
    \multirow{2}{*}{intra-process} & in-place     & \cmark & \cmark     & \xmark &\cmark \\
                                   & out-of-place & \cmark & \xmark     & \xmark &o      \\
    \multirow{2}{*}{cross-process} & in-place     & \cmark & \xmark$^a$ & \xmark &o      \\
                                   & out-of-place & \cmark & (\cmark)   & \xmark &o      \\
    \bottomrule
    \multicolumn{6}{l}{$^a$ Only works if pinned to a core}
\end{tabular}

==> tables/spectre/fc-spectre-pocs-protected.tex <==
\begin{tabular}{ccccccc}
    \toprule
                                   &              & PHT    & BTB    & RSB    & STL    \\
    \midrule
    \multirow{2}{*}{intra-process} & in-place     & \cmark & \cmark & \xmark & \xmark \\
                                   & out-of-place & \cmark & \xmark & \xmark & o      \\
    \multirow{2}{*}{cross-process} & in-place     & \cmark & \cmark & \xmark & o      \\
                                   & out-of-place & \cmark & ?      & \xmark & o      \\
    \bottomrule
\end{tabular}

==> tables/spectre/spectre-pocs-protected.tex <==
%\begin{tabularx}{\linewidth}{ccccccc}
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Variant} & \multirow{2}{*}{Platform} & \multirow{2}{*}{Thread Configuration} & \multicolumn{2}{c}{same-process} & \multicolumn{2}{c}{cross-process} \\
                                                                                \cmidrule(rl){4-5}                 \cmidrule(rl){6-7}
                     &                              &                         & in-place   & out-of-place        & in-place   & out-of-place         \\
\midrule
\multirow{2}{*}{PHT} & \multirow{1}{*}{Bare Metal}  & any                    & \noprotect & \noprotect          & \noprotect & \noprotect           \\%& none                    & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                     % &                              & \pinned(1PT)            & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                     % &                              & \pinned(2PT)            & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                       % \cmidrule(rl){2-7}
                     & \multirow{1}{*}{Firecracker} & any                   & \noprotect & \noprotect          & \noprotect & \noprotect           \\%& 1vCPU                   & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                     % &                              & 2vCPU                   & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                     % &                              & \pinned(1PT), 1vCPU     & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                     % &                              & \pinned(1PT), 2vCPU     & \noprotect & \noprotect          & \noprotect & \noprotect           \\
                     % &                              & \pinned(2PT), 2vCPU     & \noprotect & \noprotect          & \noprotect & \noprotect           \\
\midrule
\multirow{8}{*}{BTB} & \multirow{3}{*}{Bare Metal}  & none                    & \noprotect & \protects           & \protects  & \novuln$^a$          \\
                     &                              & \pinned(1PT)            & \noprotect & \protects           & \noprotect & \protects            \\
                     &                              & \pinned(2PT)            & \noprotect & \protects           & \noprotect & \protects            \\
                       \cmidrule(rl){2-7}
                     & \multirow{5}{*}{Firecracker} & 1vCPU                   & \noprotect & \protects           & \noprotect & \protects            \\
                     &                              & 2vCPU                   & \noprotect & \protects           & \noprotect & \protects            \\
                     &                              & \pinned(1PT), 1vCPU     & \noprotect & \protects           & \noprotect & \protects            \\
                     &                              & \pinned(1PT), 2vCPU     & \noprotect & \protects           & \noprotect & \protects            \\
                     &                              & \pinned(2PT), 2vCPU     & \noprotect & \protects           & \noprotect & \protects            \\
\midrule
\multirow{2}{*}{RSB} & \multirow{1}{*}{Bare Metal}  & any                    & \protects  & \protects           & \protects  & \protects            \\%& none                    & \protects  & \protects           & \protects  & \protects            \\
                     % &                              & \pinned(1PT)            & \protects  & \protects           & \protects  & \protects            \\
                     % &                              & \pinned(2PT)            & \protects  & \protects           & \protects  & \protects            \\
                     %   \cmidrule(rl){2-7}
                     & \multirow{1}{*}{Firecracker} & any                   & \protects  & \protects           & \protects  & \protects            \\%& 1vCPU                   & \protects  & \protects           & \protects  & \protects            \\
                     % &                              & 2vCPU                   & \protects  & \protects           & \protects  & \protects            \\
                     % &                              & \pinned(1PT), 1vCPU     & \protects  & \protects           & \protects  & \protects            \\
                     % &                              & \pinned(1PT), 2vCPU     & \protects  & \protects           & \protects  & \protects            \\
                     % &                              & \pinned(2PT), 2vCPU     & \protects  & \protects           & \protects  & \protects            \\
\midrule
\multirow{1}{*}{STL} & \multirow{1}{*}{Bare Metal}  & any                    & \noprotect & \novuln             & \novuln    & \novuln              \\%& none                    & \noprotect & \novuln             & \novuln    & \novuln              \\
                     % &                              & \pinned(1PT)            & \noprotect & \novuln             & \novuln    & \novuln              \\
                     % &                              & \pinned(2PT)            & \noprotect & \novuln             & \novuln    & \novuln              \\
                     %   \cmidrule(rl){2-7}
                     & \multirow{1}{*}{Firecracker} & any                    & \noprotect & \novuln             & \novuln    & \novuln              \\%& 1vCPU                   & \noprotect & \novuln             & \novuln    & \novuln              \\
                     % &                              & 2vCPU                   & \noprotect & \novuln             & \novuln    & \novuln              \\
                     % &                              & \pinned(1PT), 1vCPU     & \noprotect & \novuln             & \novuln    & \novuln              \\
                     % &                              & \pinned(1PT), 2vCPU     & \noprotect & \novuln             & \novuln    & \novuln              \\
                     % &                              & \pinned(2PT), 2vCPU     & \noprotect & \novuln             & \novuln    & \novuln              \\
\bottomrule
%\multicolumn{7}{X}{\protectskey} \\
\multicolumn{7}{p{12cm}}{\protectskey} \\
\multicolumn{7}{l}{\pinned($X$PT) --  bare metal \acs{PoC} processes/Firecracker VM vCPUs were pinned to $X$ physical sibling threads.} \\
\multicolumn{7}{l}{$X$vCPU -- the Firecracker VM has $X$ virtual CPUs.} \\
\multicolumn{7}{l}{$^a$ the \acs{PoC} does not support running without being assigned to a core.}
%\end{tabularx}
\end{tabular}

%   * Bare Metal
%       * Unpinned
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   not supported
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%       * Pinned (1)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%       * Pinned (2)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%   * Firecracker (Ubuntu 18.04, linux 5.4)
%       * Unpinned (single core)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%       * Unpinned (dual core)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%       * Pinned (1) (single core)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%       * Pinned (1) (dual core)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works
%       * Pinned (2) (dual core)
%           * PHT
%               * sa-ip:    works
%               * sa-oop:   works
%               * cp-ip:    works
%               * cp-oop:   works
%           * BTB
%               * sa-ip:    works
%               * sa-oop:   fails
%               * cp-ip:    works
%               * cp-oop:   fails
%           * RSB
%               * sa-ip:    fails
%               * sa-oop:   fails
%               * cp-ip:    fails
%               * cp-oop:   fails
%           * STL
%               * sa-ip:    works

